Analysis of the RMM-01 Market Maker

Constant function market makers(CFMMS) are a popular market design for decentralized exchanges(DEX). Liquidity providers(LPs) supply the CFMMs with assets to enable trades. In exchange for providing this liquidity, an LP receives a token that replicates a payoff determined by the trading function used by the CFMM. In this paper, we study a time-dependent CFMM called RMM-01. The trading function for RMM-01 is chosen such that LPs recover the payoff of a Black--Scholes priced covered call. First, we introduce the general framework for CFMMs. After, we analyze the pricing properties of RMM-01. This includes the cost of price manipulation and the corresponding implications on arbitrage. Our first primary contribution is from examining the time-varying price properties of RMM-01 and determining parameter bounds when RMM-01 has a more stable price than Uniswap. Finally, we discuss combining lending protocols with RMM-01 to achieve other option payoffs which is our other primary contribution.

==> includes/glossary.tex <==
%----------------------------------------------------------------------%
% Glossary File -------------------------------------------------------%
%----------------------------------------------------------------------%

% Acronyms

\newacronym{LP}{LP}{Liquidity Provider}
\newacronym{LPT}{\textsf{LPT}}{Liquidity Provider Token}
\newacronym{RMM}{RMM}{Replicating Market Maker}
\newacronym{AMM}{AMM}{Automated Market Maker}
\newacronym{EVM}{EVM}{Ethereum Virtual Machine}
\newacronym{defi}{DeFi}{Decentralized Finance}
\newacronym{tradfi}{TradFi}{Traditional Finance}
\newacronym{MEV}{MEV}{Maximal Extractable Value}
\newacronym{DEX}{DEX}{Decentralized Exchange}
\newacronym{CFMM}{CFMM}{Constant Function Market Maker}
\newacronym{CC}{CC}{Covered Call}
% \newacronym{MEV}{MEV}{Maximal (or Minor) Extractable Value}

% Glossary Entries

\newglossaryentry{Uniswap}
{
  name={Uniswap V2},
  description={A constant product market maker based exchange. Note that there has been an update to their protocol to Uniswap V3 which is described in their white paper \cite{adams_uniswap_nodate}.},
  first={\glsentrytext{Uniswap}}
}
% \newglossaryentry{CFMM}{
%     name={Constant Function Market Maker},
%     description={A automatic market maker governed by a trading function}}
\newglossaryentry{RMM-01}
{
  name={RMM-01},
  description={Primitive's implementation of a CFMM that replicates the payoff of a covered call.},
  first={\glsentrytext{RMM-01}}
}

\newglossaryentry{ERC20}
{
  name={ERC20},
  description={The standard used for creating smart contracts on the Ethereum blockchain.},
  first={\glsentrytext{ERC20}}
}
%----------------------------------------------------------------------%
